MERCURY: Accelerating DNN Training By Exploiting Input Similarity

Deep Neural Networks (DNN) are computationally intensive to train. It consists of a large number of multidimensional dot products between many weights and input vectors. However, there can be significant similarity among input vectors. If one input vector is similar to another, its computations with the weights are similar to those of the other and, therefore, can be skipped by reusing the already-computed results. We propose a novel scheme, called MERCURY, to exploit input similarity during DNN training in a hardware accelerator. MERCURY uses Random Projection with Quantization (RPQ) to convert an input vector to a bit sequence, called Signature. A cache (MCACHE) stores signatures of recent input vectors along with the computed results. If the Signature of a new input vector matches that of an already existing vector in the MCACHE, the two vectors are found to have similarities. Therefore, the already-computed result is reused for the new vector. To the best of our knowledge, MERCURY is the first work that exploits input similarity using RPQ for accelerating DNN training in hardware. The paper presents a detailed design, workflow, and implementation of the MERCURY. Our experimental evaluation with twelve different deep learning models shows that MERCURY saves a significant number of computations and speeds up the model training by an average of 1.97X with an accuracy similar to the baseline system.

==> rebuttal/MICRO22/rebut1.tex <==
We appreciate the valuable feedback from the reviewers. We submitted a revision with changes in purple color. We answer various concerns here.

Common Concerns (CC):

CC1. Why training? (Reviewer-A, B, D, E)
> We added new results in Page 1 to show that there is significant similarity in gradient vectors (up to 67%) which are used during the backward propagation. Therefore, in addition to the forward propagation, the idea of vector similarity can be exploited in the backward propagation. 

CC2. Novelty wrt [33] & [42] (Reviewer-C, E)
> There are three major differences. 
(i) Both [33] & [42] target inference only whereas Mercury targets both forward and backward propagation. 
(ii) [33] & [42] use element wise comparison to determine if input elements are similar. This is inefficient since the comparison either needs to be done serially over all elements or only within a limited number of neighboring elements. Mercury uses a well established hashing technique, RPQ, for similarity detection. RPQ can check similarity at vector granularity in constant time. RPQ is hardware-friendly and can potentially be applied to a range of hardware approximation approaches. 
(iii) Unlike Mercury, [33] & [42] require a new dataflow in the accelerator and cannot be used on top of an existing dataflow.

CC3. More networks and layers. (Reviewer-A, D, E)
> We added 3 more networks. We added support for fully connected and attention layers (Page-8). We could not show the complete the results of these new layers in the revision.

CC4. Convergence? (Reviewer-A, C)
> We may need to train for more epochs to reach the original accuracy. However, similar to prior research, we argue that 0.7% accuracy degradation should be acceptable in most applications. We added a discussion in Page-10.

Reviewer-A:

A1. Experimental details?
> We added the details in Page-9.

Reviewer-B:
B1. Hash function analysis?
> We added a characteristic analysis in Page-3.

B2. Compare against Eyeriss & Procrustes?
> Our baseline system is Eyeriss. All the speed ups are calculated wrt that. We feel that Procrustes and Mercury has different goals - one is to handle sparsity (presumably to support resource constrained environments) and the other is to speed up computations. Therefore, we did not compare against Procrustes.

B3. Oracle cache results?
>In average is only 8\% faster.

B4. Increasing PE instead?
>The proposed idea has 13.5\% power overhead and number of PE = 168. In baseline design we can have 25 more PEs which will give us only 16\% acceleration in training.

Reviewer-C:
C1. Increased memory access?
> We agree that Mercury requires accesses to MCache memory. However, MCache consists of on-chip memory. Therefore, there is no new access to off-chip memory.

C2. Why better than unlimited similarity?
> In unlimited similarity, if two elements are completely similar than computations of the second element can be saved. Since this is element-wise similarity, it saves less computations than vector-wise similarity such as Mercury.

C3. High hit rate but low computation reduction?
> In the previous version, we used the term hit in a different sense than the traditional cache-related term. Therefore, we redrawn Figure 17(a) with terms consistent with prior sections.

C4. Hardware per module?
>We are collecting the data and we will include it in final version.

Reviewer-D:
D1. Compare with software approaches?
> Software approaches report speed up with respect to a software-based baseline. In addition, software approaches have flexibility to exploit similarity at different granularity (e.g., single vector, sub-vector, multiple channels, across inputs, etc.) leading to a greater scope for computation saving. Prior software approaches report saving 60% computations leading to a 2.5x speed up. However, that number is based on only 3 small networks.

D2. Improvement from poor baseline?
> Results from software approaches suggest that the performance benefit comes from the computation reuse algorithm itself, not from poor FPGA baseline.

D3. Frequency?
> 130MHz

D4. Unlimited zero pruning?
> We modeled this approach as an ideal case where we save any computation involving zero without any regard to resource constraints.

D5. Deep dive case?
> We showed VGG in the revision (Page-12).

D6. MCache hit rate?
>In average the hit rate is almost 50\% for layers with larger inputs and for layers with smaller inputs less than 27 we don't have Cache capacity miss but since inputs are small so the hit-rate is about 30\%.

Reviewer-E:

E1. Why no cache replacement?
> If a signature has a hit with a previous signature in the cache, the hitmap will contain HIT. If we allow later signatures to replace earlier signatures, we need to reinitialize hitmap with new values. This is of-course feasible but will make the design more complex. So, we choose not to replace existing signatures. Compared to an ideal design with unlimited signatures, the default design is only 8\% slower.

E2. Analysis on signature length?
> Signature length starts at 20 and increases up to 30 for VGG and ResNet. Over 30, the computation reuse opportunity significantly diminishes (because most vectors get identified as distinct). So, we did not go beyond 30.

E3. Model selection?
> We selected models that can be trained to completion with our hardware and software testbed.







==> related.tex <==
There has been a considerable amount of efforts on CNN acceleration and their efficiency~\cite{eyeriss, dcompress, tdash, tfe, perforate, binarynet, inq, cnvlutin}.
%, which can be split into two (2) main categories: model optimization and computational reuse.
%\subsection{Model Optimization}
%Research in this area optimizes either the model's weights or the model's architecture, notably weight quantization~\cite{binarynet, inq}, sparsity exploitation~\cite{tdash, cnvlutin} or model compression~\cite{tfe, dcompress}.
Courbariaux et al.~\cite{binarynet} propose BinaryNet, a network whose weights are quantized to either +1 or -1. Due to these binary weights, all arithmetic calculations in the network can be replaced by bitwise operations, thus significantly reducing the memory footprint of the model. 
%One drawback of this approach is accuracy loss. On ImageNet classification task, the model achieves 36.1\% and 47.1\% top-1 accuracy for AlexNet and GoogleNet, respectively.
Another line of work attempts to exploit the sparsity within the model architecture. Mahmoud et al.~\cite{tdash} find out that the multiply-accumulate (MAC) operations account for a significant amount of energy consumption in model training. In a MAC operation, if any of the operands is zero, it can be safely ignored. As such, they propose TensorDash, a hardware scheduler that can efficiently find and skip unnecessary MAC computations. 
%The speedup depends on the sparsity of the network. The more zeros occur in the backward and forward passes, the more speedup TensorDash will get.
Albericio et al.~\cite{cnvlutin} show that almost half of the calculations within the convolutional layers involve multiplying with zero. As such, they present Cnvlutin, a CNN-centric hardware accelerator that can detect and eliminate most of these unnecessary computations. 
%Cnvlutin decouples the input and output between two consecutive convolutional layers. Intermediate results are recorded in a special data format, which allows the succeeding layer to read only non-zero values. In this way, zero neurons are nullified at the output of the preceding layer at runtime. In image classification task, Cnvlutin increases the overall performance by 52\% without sacrificing any accuracy loss.
Han et al. propose Deep Compression (DC)~\cite{dcompress}, a holistic solution that combines model pruning and weight quantization. At the beginning, DC removes all connections whose weights are smaller than a preset threshold. The remaining weights are then quantized and encoded. 
%Experiment results show that this approach can reduce the memory footprint of AlexNet and VGG-16 by 35x and 49x, with negligible accuracy loss. Deep Compression is most effective on fully connected layers, with 96\% amount of the weights are pruned in VGG-16.

%\subsection{Data and Computational Reuse}
%Research in this direction exploits the fact that there are a lot of data repetition in the convolution computation. As such, they attempt to reuse different kind of intermediate data during the CNN inference and training. 

%Eyeriss~\cite{eyeriss} attempts to minimize data movement by reusing input data including filter weights and feature maps. The underlying dataflow, called Row Stationary (RS), increases the energy efficiency of AlexNet up to 2.5x. Unlike other dataflows, RS optimizes both data reuse and partial sum accumulation cost, thus gives more efficiency gain.

%Hegde et al.~\cite{ucnn} propose UCNN accelerator architecture. UCNN exploits the fact that current weight quantization techniques produce a lot of weight repetitions in the CNN model. As such, we can reuse the result, reduce the number of computations and also the model memory footprint. In the core of UCNN is the factorized dot product dataflow and activation group reuse. Factorized dot product first detects and groups the inputs that are multiplied with the same weight into \textit{activation groups}. Each group is then summed and multiplied with the common weight. As a result, the number of multiplications is reduced to one per group. UCNN further exploits the repetition across different filters using activation group reuse. If there are overlapped elements between activation group of two filters, these common elements can be reused across two filters. 

%Ning et al.~\cite{dreuse} propose Adaptive Deep Reuse (ADR) to exploit computational reuse to accelerate the CNN training process. Unlike UCNN, ADR focuses on finding repetitions in the input data, instead of the model weights, of the convolutional layer. ADR exploits the fact that there are a considerable amount of similarities in the input matrix. Input matrix is first factorized into neuron vectors. Similar neuron vectors are put into clusters, and only the center vector of each cluster is multiplied with the filter weight. All other neuron vectors in the group reuse this result. ADR opts for Locality Sensitive Hashing (LSH) as its clustering method.

==> taxonomy.tex <==
Exploiting computational similarity is one way to optimize computations. We propose a taxonomy of computation optimization techniques based on time, data, and granularity of computation optimization. Table~\ref{table-taxonomy} shows the taxonomy.
%categorizes prior computational optimizations based on three major characteristics: time, data, and granularity. 
As an example, Cnvultin~\cite{cnvlutin} tries to detect zero inputs to reduce unnecessary multiplications in the inference process, thus it is put in Inference/Input/Single Element. Deep Compression~\cite{dcompress} tries to quantize model weights to reduce the inference computational cost, therefore it is categorized as an Inference/Filter/Multiple Elements technique. 

There are techniques that belong to multiple categories. For instance, SCNN~\cite{scnn} exploits the sparsity in both weights and activations, therefore it falls into both Input and Filter classes.
\scheme\ falls under the category Training/Input/Multiple Elements. Although Ning et al.~\cite{adaptivedeepreuse} is in the same category, its scope is limited to software %to optimize software implementations 
%machine learning libraries 
as opposed to a hardware accelerator (more on this in Section~\ref{sec-comp-reuse}). 
%Thus, \scheme\ is the first work in its category that accelerates hardware.
%Note that those approaches that optimize the training process can also work for model inference. For example, BinaryNet~\cite{binarynet} is technically an extreme quantization technique that works for both training and inference.

\begin{table}[h!]
\centering
%\scriptsize
\scalebox{0.8}{
\begin{tabular}{|| c | c | l | c ||} 
 \hline\hline
 Time & Data & Granularity & Examples \\ [0.5ex] 
 \hline\hline
 Inference & Input  & Single Element only    & ~\cite{cnvlutin}~\cite{scnn}*\\
           &        & Multiple Elements      & ~\cite{snapea}~\cite{uspe}~\cite{dreuse}~\cite{eie}*~\cite{riera-reuse} \\[1ex]
           & Filter & Single Element only    & ~\cite{scnn}*~\cite{tdash}* \\
           &        & Multiple Elements      & ~\cite{ucnn}~\cite{inq}~\cite{tfe}~\cite{eie}* \\[1ex]
 \hline
 Training  & Input  & Single Element only    & None \\
           &        & Multiple Elements      & {\bf \scheme},~\cite{adaptivedeepreuse} \\[1ex]
           & Filter & Single Element only    & ~\cite{eager-prune}~\cite{tdash}* \\
           &        & Multiple Elements      & ~\cite{binarynet}~\cite{perforate}~\cite{dcompress} \\[1ex]
 \hline\hline
\end{tabular}}
\caption{Categories of computation optimization techniques. Any work with * belongs to multiple categories}
\label{table-taxonomy}
\vspace{-0.6cm}
\end{table}

%\footnotetext{Work that belongs to multiple categories.}
